M$^2$Hub: Unlocking the Potential of Machine Learning for Materials Discovery

We introduce M$^2$Hub, a toolkit for advancing machine learning in materials discovery. Machine learning has achieved remarkable progress in modeling molecular structures, especially biomolecules for drug discovery. However, the development of machine learning approaches for modeling materials structures lag behind, which is partly due to the lack of an integrated platform that enables access to diverse tasks for materials discovery. To bridge this gap, M$^2$Hub will enable easy access to materials discovery tasks, datasets, machine learning methods, evaluations, and benchmark results that cover the entire workflow. Specifically, the first release of M$^2$Hub focuses on three key stages in materials discovery: virtual screening, inverse design, and molecular simulation, including 9 datasets that covers 6 types of materials with 56 tasks across 8 types of material properties. We further provide 2 synthetic datasets for the purpose of generative tasks on materials. In addition to random data splits, we also provide 3 additional data partitions to reflect the real-world materials discovery scenarios. State-of-the-art machine learning methods (including those are suitable for materials structures but never compared in the literature) are benchmarked on representative tasks. Our codes and library are publicly available at https://github.com/yuanqidu/M2Hub.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{We do not anticipate any negative societal impacts of the work as materials discovery is essential to many fundamental areas such as sustainability, energy, healthcare, etc.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Appendix~\ref{sec:exp_detail}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{sec:exp_detail}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We did not run all experiments for multiple times mainly because of the lack of computational resources. We did observe the results not change much across runs.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec:benchmark}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{sec:dataset}.}
  \item Did you mention the license of the assets?
    \answerYes{See Section~\ref{sec:dataset}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{For the code we release with this project \url{https://github.com/yuanqidu/M2Hub}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See Section~\ref{sec:dataset}, by license.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> deprecated.tex <==
\begin{table}
\begin{center}
\caption{\yq{structure, composition only}}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{cccccccccc}
\toprule
Source & Subset & Materials type & Dim (real) & Dim (PBC) & Property & Prop. type & Task type & \# data & Method\\
\hline 
\multirow{15}{*}{MP~\cite{jain2013commentary}}
& \multirow{13}{*}{MatBench} & Inorganic bulk & 3D & 3D & Band gap & Electronic & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Metallicity & Electronic & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Band gap (exp) & Electronic & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Metallicity (exp) & Electronic & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Bulk modulus & Mechanical & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Shear modulus & Mechanical & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Steel yield strength & Mechanical & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Bulk metallic glass formation & Stability & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Formation energy & Stability & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Formation energy of Perovskite cell & Stability & Scalar &  \\
& & Inorganic bulk & 3D & 2D & Exfoliation energy & Stability & Scalar &  \\
& & Inorganic bulk & 3D & 3D & Freq. at last phonon PhDOS peak & Optical & Scalar &  \\
\cmidrule{3-9}
& QMOF & Metal-organic framework & \\
\cmidrule{3-9}
& Ours & Inorganic bulk & \\
\cmidrule{2-9}
\multirow{1}{*}{OC~\cite{chanussot2021open}}
& None & Catalyst surface & \\
\cmidrule{2-9}
\multirow{1}{*}{OMDB~\cite{borysov2017organic}}
& None & Organic crystal & Band gap &  & Scalar & 12,500\\
\cmidrule{2-9}
\multirow{2}{*}{JARVIS~\cite{choudhary2020joint}}
& JARVIS-DFT3D & Bulk (?) \\
& JARVIS-EDOS\_PDOS & (?) \\
\cmidrule{2-9}
\multirow{2}{*}{Materials Cloud~\cite{talirz2020materials}}
& MC3D & Inorganic bulk  & \\
& MC2D & Low-d materials & \\
\cmidrule{2-9}
\multirow{1}{*}{tmQM~\cite{balcells2020tmqm}}
& None & Molecule & \\
\cmidrule{2-9}
\multirow{1}{*}{COD~\cite{gravzulis2012crystallography}}
& None & Organic crystal & None & None & None & \\
% \cmidrule{2-9}
% \multirow{1}{*}{C2DB~\cite{gjerding2021recent}} 
% & None & Low-d materials & \\
% \cmidrule{2-9}
% \multirow{1}{*}{HPOV~\cite{lopez2016harvard}} 
% & None & (?) & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}
